Exploiting Correlations Between Contexts and Definitions with Multiple Definition Modeling

Definition modeling is an important task in advanced natural language applications such as understanding and conversation. Since its introduction, it focus on generating one definition for a target word or phrase in a given context, which we refer to as Single Definition Modeling (SDM). However, this approach does not adequately model the correlations and patterns among different contexts and definitions of words. In addition, the creation of a training dataset for SDM requires significant human expertise and effort. In this paper, we carefully design a new task called Multiple Definition Modeling (MDM) that pool together all contexts and definition of target words. We demonstrate the ease of creating a model as well as multiple training sets automatically. % In the experiments, we demonstrate and analyze the benefits of MDM, including improving SDM's performance by using MDM as the pretraining task and its comparable performance in the zero-shot setting.

==> Related_Work.tex <==
\section{Related Work}
The first study on definition modeling is proposed by \citet{DBLP:conf/aaai/NorasetLBD17}, which uses word embeddings to generate corresponding word definitions by an RNN-based sequence-to-sequence model. 
%They also attempted to append hypernym embeddings but did not get extra profits.
However, the problem of polysemes cannot be addressed by only exploiting word embedding. 
%Some works introduced additional information to help model polysemes, such as the context where a word appears. 
\citet{DBLP:conf/ijcnlp/NiW17} first attempted to model local contexts of a word for Internet slang explanation generation. Following this work, many works argued utilizing contexts could help generate multiple definitions for polysemes.  \citet{DBLP:conf/acl/GadetskyYV18} employed Adaptive Skip-Gram model \cite{pmlr-v51-bartunov16} to learn the required number of vector representations for each polyseme. 
% The definition generation will be conditioned on the Adaptive Skip-gram vector representations. 
% Xsense proposed by \citet{chang2018xsense} also investigate the word embeddings by pinning down a specific dimension in the sparse word representation which maintain one of the senses of a word. 
% And then they applied a RNN to generate definitions for the corresponding word embeddings. 
\citet{DBLP:conf/naacl/IshiwatariH0NST19} created a Wikipedia dataset that takes the descriptions of a word as target and uses the sentences referring to the target item from Wikipedia articles as contexts. 
%It also uses both local and global contexts for description generation. 
Nevertheless, \citet{DBLP:conf/acl/GadetskyYV18,chang2018xsense, DBLP:conf/naacl/IshiwatariH0NST19,li-etal-2020-explicit,washio-etal-2019-bridging, chang-chen-2019-word} mainly used definition modeling to obtain static sense embedding from contexts, which did not fully utilize the context information and the sense embeddings are not contextual.

Recently, more and more definition modeling methods explore Transformer \cite{DBLP:journals/corr/VaswaniSPUJGKP17} based pretrained natural language generation models \cite{DBLP:journals/corr/abs-1911-05715, DBLP:conf/acl/LewisLGGMLSZ20,raffel2020exploring, DBLP:journals/corr/abs-1810-04805} to generate definitions given the contexts. Generationary \cite{DBLP:conf/emnlp/BevilacquaMN20} leveraged BART to generate corresponding gloss for the span in contexts where the target word appears. 
%Additionally, Generationary was assessed on Word Sense Disambiguation (WSD) and Word in Context (WiC) task to prove the potential of Generationary in discriminative tasks. 
\citet{DBLP:journals/corr/abs-2010-03124} proposed VCDM and introduced a continuous latent variable to explicitly model the underlying relationship between context and definition. 
%Variational inference was applied for estimation and contextualized word embeddings was leveraged for improved performance. 
Some works also studied other aspects of definition generation. \cite{DBLP:conf/emnlp/HuangKA21} utilized a re-ranking mechanism to model specificity in definitions. 
%and generality of output generated by T5 \cite{raffel2020exploring}. 
\citet{DBLP:conf/acl/KongCZYY22} emphasized simplification by proposing a SimpDefiner model which integrated three sub-tasks of definition generation with a weight sharing mechanism. Note that none of the aforementioned works attempted generating multiple definitions of a word at one time and exploiting coarse contexts possibly misaligned with the target definitions. %Although Wikipedia dataset \cite{DBLP:conf/naacl/IshiwatariH0NST19} also used open-domain articles, it is still regard each context as an input but not inputs. 
Our work not only proposes a novel multiple definition modeling task but also constructs a new dataset for MDM with open-domain contexts.

==> Results.tex <==
\section{Analysis and Discussion}
\label{sec:analysis}

\paragraph{Performance on Novel Sense Generation}
We evaluated the \emph{Novel Sense Generation} performance of generating out-of-sense-inventory definitions from SDM and MDM models. As described in Section~\ref{subsec:experimental-setup}, we created datasets based on the Oxford dataset by holding out $D$ definitions with their corresponding contexts (usage examples in Oxford). With $D=\{1,2,3\}$, we created three datasets: DEL-1, DEL-2 and DEL-3.

% For example, if there are three definitions in different senses with their corresponding contexts for a word, we randomly select one definitions and add the selected definitions with their contexts to a holdout set which will be used as test data later. For the two definitions and their contexts will be used for training. The same operation will be conduct for selecting two definitions. The first dataset is denoted as DEL\_1\_DEF while the second is named as DEL\_2\_DEF. 
Note that the format of data for training SDM and MDM models is quite different. We took pairs composed of a single definition and its corresponding usage example for SDM training; whereas, we used concatenated definitions and concatenated contexts for MDM training. To make a fair comparison, we concatenated the predicted definitions by 
BART-SDM (i.e., BART trained on the SDM data)
with \verb!<sep>! and conducted the same operation on the corresponding gold definitions to calculate metric scores. No operations are needed for MDM predictions and references. 

\begin{table}[htpb]
\centering
\scalebox{0.8}{
\begin{tabular}{@{}c|l|cccc@{}}
\toprule[2pt]
\textbf{DATA} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{R1} & \textbf{R2} & \textbf{RL} & \textbf{BS} \\ \midrule
\multirow{2}{*}{\textbf{DEL\_1}} & BART-SDM & 21.72          & 6.59          & 22.67          & 86.82          \\
                                & BART-MDM & \textbf{22.78} & \textbf{6.82} & \textbf{24.34} & \textbf{87.42} \\ \midrule
\multirow{2}{*}{\textbf{DEL\_2}} & BART-SDM & 27.46          & 7.33          & 26.91          & 86.63          \\
                                & BART-MDM & \textbf{27.96} & \textbf{8.35} & \textbf{28.81} & \textbf{88.10} \\ \midrule
\multirow{2}{*}{\textbf{DEL\_3}} & BART-SDM & 27.04          & 7.90          & \textbf{26.58} & 85.82          \\
                                & BART-MDM & \textbf{33.56} & \textbf{9.21} & 26.34          & \textbf{86.23} \\ \bottomrule[2pt]
\end{tabular}
}
\caption{Performance on \emph{Novel Sense Generation} as generating new definitions that are out of the sense inventory, given contexts. Models were trained on dataset DEL-$D$, which was created through holding out $D$ definitions and contexts for each word in an SDM benchmark, using the remaining data for training and the holdout set for testing. BART-SDM denotes finetuning the facebook/bart-base model on the DEL-$D$ dataset in the SDM format while BART-MDM denotes finetuning facebook/bart-base on DEL-$D$ in the MDM format. The evaluation metrics are the same as in Table \ref{table_main}.}
\label{table_ms}
\end{table}

\input{case_study}



\begin{table}[htpb]
\centering
\scalebox{0.8}{
\begin{tabular}{@{}c|c c@{}}
\toprule
\textbf{Model} & \textbf{Intra 2$\uparrow$} & \textbf{Inter 2$\uparrow$} \\ \midrule
BART & 39.05 & 99.25 \\
BART+word & 40.21 & 99.22 \\
BART+syn  & {\ul \textbf{41.07}} & 99.08 \\
BART+hyp & 40.77 & {\ul \textbf{99.33}} \\ \bottomrule
\end{tabular}}
\caption{Distinct-N scores between predicted and gold definitions by different models.  Intra 2 denotes sentence intra Distinct-N while Inter 2 denotes sentence inter Distinct-N. The best results are underlined and in bold.}
\label{table_distinct}
\end{table}


Table \ref{table_ms} shows that on all three datasets, a BART model trained on data in the MDM format (denoted by BART\_MDM) performs better than BART trained on the SDM format (denoted by BART\_SDM), with the only exception as BART\_SDM outperforms BART\_MDM on ROUGE\_L on the DEL-3 dataset.  In contrast, the predictions of BART-SDM would not have the same issue since we concatenate the predictions by \verb!<sep>!. That is, BART-MDM cannot take advantage of the experiment settings since the error of special tokens will be taken into account as well. In general, BART-MDM indeed performs better on generating definitions that are out of the sense inventory and shows the potential of the MDM task to help the model learn novel sense generation capability. We also listed some generated definitions by BART-SDM and BART-MDM in Table \ref{tabel_case_study} and Table \ref{tabel_case_for_del}.
The quality of definitions in DEL-1 test set is better than DEL-2 since prediction for the latter is more challenging. MDM could generate more abstractive definitions which are highly related to the sense in their contexts. For example, for ``Japanese'', the definition predicted by SDM is also reasonable but is irrelevant to the context. As for ``ban'', SDM heavily relies on the context and predicts "the act of smoking" since there is a "smoking" in context. However, MDM generates the correct definition for the first context which is "prevent (someone) from doing something".  
From these cases, we could observe that BART-MDM is able to summarize the semantics of a word in its contexts and generate more reasonable definitions. \par
%, also illustrating the potential of MDM task to generate new definitions based on the contexts. 

%We also listed some predicted results by BART-SDM and BART-MDM in Table \ref{tabel_case_study} and Table \ref{tabel_case_for_del}. The quality of definitions in DEL\_1\_DEF test data is better than DEL\_2\_DEF since the prediction for the latter test data is more challenging. But MDM could generate more abstractive definitions which are highly related to the sense in their contexts. For example, word 'japanses', the definition predicted by SDM is also reasonable but is irrelevant to the context. As for "ban", the output of SDM predicted heavly relied on the contexts, predicting "the act of smoking" since there is a "smoking" in context. However, MDM could produce the meaning of "ban" in the first context which is "prevent (someone) from doing something".  From these cases, we could observe that BART-MDM is able to summary the semantics of the word in its contexts and give a more convincing definitions. \par




% However, as for deleting 3 definitions, the size training data for SDM and MDM has a big discrepancy inducing the training for MDM is insufficient. We argue that is why the  \par 
\paragraph{Diversity Evaluation} We evaluate the diversity between generated definitions and gold definitions. We adopt Distinct-N as the metric and report the intra and inter 2-gram diversity in Table \ref{table_distinct}. The diversity of definitions generated by BART pretrained on MDM exceeds that of the baseline BART model, which shows that the auxiliary task and diversity loss could improve the diversity of multiple definition generations. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\linewidth]{EMNLP 2022/image/sense_number.png}
%     \caption{Effect of number of senses in target words.}
%     \label{fig:sense_number}
% \end{figure}






==> case_study.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table*}[htbp]
% \renewcommand{\arraystretch}{0.9}
% \scalebox{0.6}{

% \begin{tabular}{@{}llll@{}}
% \toprule[2pt]
% \multicolumn{4}{c}{\textbf{DEL 1}} \\ \midrule
% \multicolumn{1}{l|}{\textbf{WORD}} &
%   \multicolumn{1}{l|}{wad} &
%   \multicolumn{1}{l|}{\textbf{WORD}} &
%   privy \\ \midrule
% \multicolumn{1}{l|}{\textbf{CONTEXT}} &
%   \multicolumn{1}{l|}{<w> wad <w> he used a wad of cotton to wipe the counter} &
%   \multicolumn{1}{l|}{\textbf{CONTEXT}} &
%   <w> privy <w> privy to the details of the conspiracy \\ \midrule
% \multicolumn{1}{l|}{\textbf{DEFINITION}} &
%   \multicolumn{1}{l|}{a small mass of soft material} &
%   \multicolumn{1}{l|}{\textbf{DEFINITION}} &
%   informed about something secret or not generally known \\ \midrule
% \multicolumn{1}{l|}{\textbf{SDM\_PRED}} &
%   \multicolumn{1}{l|}{a small piece of something} &
%   \multicolumn{1}{l|}{\textbf{SDM\_PRED}} &
%   completely or completely \\ \midrule
% \multicolumn{1}{l|}{\textbf{MDM\_PRED}} &
%   \multicolumn{1}{l|}{a small piece of cloth} &
%   \multicolumn{1}{l|}{\textbf{MDM\_PRED}} &
%   to be aware of \\ \midrule \midrule
% \multicolumn{1}{l|}{\textbf{WORD}} &
%   \multicolumn{1}{l|}{height} &
%   \multicolumn{1}{l|}{\textbf{WORD}} &
%   want \\ \midrule
% \multicolumn{1}{l|}{\textbf{CONTEXT}} &
%   \multicolumn{1}{l|}{<w> height <w> at the height of her career} &
%   \multicolumn{1}{l|}{\textbf{CONTEXT}} &
%   <w> want <w> for want of a nail the shoe was lost \\ \midrule
% \multicolumn{1}{l|}{\textbf{DEFINITION}} &
%   \multicolumn{1}{l|}{the highest level or degree attainable} &
%   \multicolumn{1}{l|}{\textbf{DEFINITION}} &
%   the state of needing something that is absent or unavailable \\ \midrule
% \multicolumn{1}{l|}{\textbf{SDM\_PRED}} &
%   \multicolumn{1}{l|}{the highest point} &
%   \multicolumn{1}{l|}{\textbf{SDM\_PRED}} &
%   the property of being lost \\ \midrule
% \multicolumn{1}{l|}{\textbf{MDM\_PRED}} &
%   \multicolumn{1}{l|}{the highest stage of development} &
%   \multicolumn{1}{l|}{\textbf{MDM\_PRED}} &
%   a desire for something \\ \midrule[2pt]
% \multicolumn{4}{c}{\textbf{DEL 2}} \\ \midrule
% \multicolumn{1}{l|}{\textbf{WORD}} &
%   \multicolumn{1}{l|}{blind} &
%   \multicolumn{1}{l|}{\textbf{WORD}} &
%   acute \\ \midrule
% \multicolumn{1}{l|}{\textbf{CONTEXT}} &
%   \multicolumn{1}{l|}{<w> blind <w> he waited impatiently in the blind <sep> blind hatred} &
%   \multicolumn{1}{l|}{\textbf{CONTEXT}} &
%   <w> acute <w> acute appendicitis <sep> acute pain \\ \midrule
% \multicolumn{1}{l|}{\textbf{DEFINITION}} &
%   \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}a hiding place sometimes used by hunters especially duck hunters \\<sep> not based on reason or evidence\end{tabular}} &
%   \multicolumn{1}{l|}{\textbf{DEFINITION}} &
%   \begin{tabular}[c]{@{}l@{}}having or experiencing a rapid onset and short but severe course\\ <sep> extremely sharp or intense\end{tabular} \\ \midrule
% \multicolumn{1}{l|}{\textbf{SDM\_PRED}} &
%   \multicolumn{1}{l|}{a person who is blind <sep> not aware of} &
%   \multicolumn{1}{l|}{\textbf{SDM\_PRED}} &
%   keenly aware <sep> lacking in resources \\ \midrule
% \multicolumn{1}{l|}{\textbf{MDM\_PRED}} &
%   \multicolumn{1}{l|}{unable to see <sep> unable to perceive} &
%   \multicolumn{1}{l|}{\textbf{MDM\_PRED}} &
%   pain or discomfort <sep> severe \\ \midrule \midrule
% \multicolumn{1}{l|}{\textbf{WORD}} &
%   \multicolumn{1}{l|}{couple} &
%   \multicolumn{1}{l|}{\textbf{WORD}} &
%   blue \\ \midrule
% \multicolumn{1}{l|}{\textbf{CONTEXT}} &
%   \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}<w> couple <w>  he 's coming for a couple of days \\ <sep>  can we couple these proposals ?\end{tabular}} &
%   \multicolumn{1}{l|}{\textbf{CONTEXT}} &
%   \begin{tabular}[c]{@{}l@{}}<w> blue <w> he had eyes of bright blue \\ <sep>  October 's bright blue weather " - Helen Hunt Jackson\end{tabular} \\ \midrule
% \multicolumn{1}{l|}{\textbf{DEFINITION}} &
%   \multicolumn{1}{l|}{a small indefinite number <sep> to link together} &
%   \multicolumn{1}{l|}{\textbf{DEFINITION}} &
%   \begin{tabular}[c]{@{}l@{}}resembling the color of the clear sky in the daytime \\ <sep> of the color intermediate between green and violet\end{tabular} \\ \midrule
% \multicolumn{1}{l|}{\textbf{SDM\_PRED}} &
%   \multicolumn{1}{l|}{of or belonging to a married couple <sep> to combine} &
%   \multicolumn{1}{l|}{\textbf{SDM\_PRED}} &
%   bright and clear <sep> not bright \\ \midrule
% \multicolumn{1}{l|}{\textbf{MDM\_PRED}} &
%   \multicolumn{1}{l|}{a group of people <sep> to combine into one} &
%   \multicolumn{1}{l|}{\textbf{MDM\_PRED}} &
%   the color of the sky <sep> characterized by bright colors \\ \bottomrule[2pt]
% \end{tabular}

% }
% \caption{This table listed generated definitions from BART-SDM and BART-MDM on incomplete datasets in Quantitative Analysis on Generated Multiple Definition.}
% \label{tabel_case_study}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table*}[htpb]
% \centering
% \scalebox{0.5}{
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{tabular}{@{}llll@{}}
% \toprule[2pt]
% \multicolumn{4}{c}{\textbf{DEL 1}} \\ \midrule
% \multicolumn{1}{l|}{\textbf{WORD}} &
%   \multicolumn{1}{l|}{japanese} &
%   \multicolumn{1}{l|}{\textbf{WORD}} &
%   submerse \\ \midrule
% \multicolumn{1}{l|}{\textbf{CONTEXT}} &
%   \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}<w> japanese <w> unlike the belgians , americans and japanese ,\\ the british have no heritage of adult comic books .\end{tabular}} &
%   \multicolumn{1}{l|}{\textbf{CONTEXT}} &
%   \begin{tabular}[c]{@{}l@{}}<w> submerse <w>  this is one of the great strengths of the play ; \\ though it may at times seem over-determined , and perhaps even obvious , \\ the audience is entirely submersed in the characters and their worlds .\end{tabular} \\ \midrule
% \multicolumn{1}{l|}{\textbf{DEFINITION}} &
%   \multicolumn{1}{l|}{a native or inhabitant of japan , or a person of  japanese descent .} &
%   \multicolumn{1}{l|}{\textbf{DEFINITION}} &
%   submerge \\ \midrule
% \multicolumn{1}{l|}{\textbf{SDM\_PRED}} &
%   \multicolumn{1}{l|}{the mandarin language of japan.} &
%   \multicolumn{1}{l|}{\textbf{SDM\_PRED}} &
%   make rigid or rigid \\ \midrule
% \multicolumn{1}{l|}{\textbf{MDM\_PRED}} &
%   \multicolumn{1}{l|}{a native or inhabitant of japan.} &
%   \multicolumn{1}{l|}{\textbf{MDM\_PRED}} &
%   become immersed in \\ \midrule \midrule
% \multicolumn{1}{l|}{\textbf{WORD}} &
%   \multicolumn{1}{l|}{brink} &
%   \multicolumn{1}{l|}{\textbf{WORD}} &
%   humbleness \\ \midrule
% \multicolumn{1}{l|}{\textbf{CONTEXT}} &
%   \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}<w> brink <w> at last he implored edgar to guide him to the \\ brink of a cliff so that he could throw himself off .\end{tabular}} &
%   \multicolumn{1}{l|}{\textbf{CONTEXT}} &
%   w humbleness w  not everyone regards humility as a virtue \\ \midrule
% \multicolumn{1}{l|}{\textbf{DEFINITION}} &
%   \multicolumn{1}{l|}{the extreme edge of land before a steep slope or a body or water} &
%   \multicolumn{1}{l|}{\textbf{DEFINITION}} &
%   a disposition to be humble ; a lack of false pride \\ \midrule
% \multicolumn{1}{l|}{\textbf{SDM\_PRED}} &
%   \multicolumn{1}{l|}{the point at which something is likely to happen} &
%   \multicolumn{1}{l|}{\textbf{SDM\_PRED}} &
%   regard as worthy or worthy of consideration \\ \midrule
% \multicolumn{1}{l|}{\textbf{MDM\_PRED}} &
%   \multicolumn{1}{l|}{the edge of something} &
%   \multicolumn{1}{l|}{\textbf{MDM\_PRED}} &
%   the quality of being humble \\ \midrule[1.5pt]
% \multicolumn{4}{c}{\textbf{DEL 2}} \\ \midrule
% \multicolumn{1}{l|}{\textbf{WORD}} &
%   \multicolumn{1}{l|}{snitch} &
%   \multicolumn{1}{l|}{\textbf{WORD}} &
%   placement \\ \midrule
% \multicolumn{1}{l|}{\textbf{CONTEXT}} &
%   \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}<w> snitch <w> he believes in the value of student snitches , parental conferences , \\ and long hot showers in the faculty lounge . <sep>  trey kicked \\ at it as he snitched a chocolate chip cookie from blake 's lunch .\end{tabular}} &
%   \multicolumn{1}{l|}{\textbf{CONTEXT}} &
%   \begin{tabular}[c]{@{}l@{}}<w> placement <w> traders in cleckheaton are being offered the help of \\ special-needs teenagers on work placements . <sep> students would also \\ go on more work experience placements and local business people would \\ visit the school to discuss their experiences and give advice .\end{tabular} \\ \midrule
% \multicolumn{1}{l|}{\textbf{DEFINITION}} &
%   \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}a hiding place sometimes used by hunters especially duck hunters \\ <sep>  not based on reason or evidence\end{tabular}} &
%   \multicolumn{1}{l|}{\textbf{DEFINITION}} &
%   \begin{tabular}[c]{@{}l@{}}the action of finding a home , job , or school for someone \\ <sep> the temporary posting of someone in a workplace to enable them to \\ gain work experience\end{tabular} \\ \midrule
% \multicolumn{1}{l|}{\textbf{SDM\_PRED}} &
%   \multicolumn{1}{l|}{a person who is blind <sep> not aware of} &
%   \multicolumn{1}{l|}{\textbf{SDM\_PRED}} &
%   the action of sampling something <sep> the way in which something is arranged \\ \midrule
% \multicolumn{1}{l|}{\textbf{MDM\_PRED}} &
%   \multicolumn{1}{l|}{unable to see <sep> unable to perceive} &
%   \multicolumn{1}{l|}{\textbf{MDM\_PRED}} &
%   a person's place of employment <sep> a place for someone to do something \\ \midrule
% \multicolumn{1}{l|}{\textbf{WORD}} &
%   \multicolumn{1}{l|}{ban} &
%   \multicolumn{1}{l|}{\textbf{WORD}} &
%   mope \\ \midrule
% \multicolumn{1}{l|}{\textbf{CONTEXT}} &
%   \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}<w> ban <w> smoking is banned in this building <sep> the subject is \\ banned from our interview because the case has still to come to court .\end{tabular}} &
%   \multicolumn{1}{l|}{\textbf{CONTEXT}} &
%   \begin{tabular}[c]{@{}l@{}}<w> mope <w> everyone seemed to have a good time , even fiona , who was \\ apparently trying to get over having the mopes whenever she was not the \\ direct focus of albert 's attention . <sep> i moped around the house for \\ most of the weekend , wishing scott was with me .\end{tabular} \\ \midrule
% \multicolumn{1}{l|}{\textbf{DEFINITION}} &
%   \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}prohibit especially by legal means or social pressure \\ <sep> officially or legally prohibit ( something )\end{tabular}} &
%   \multicolumn{1}{l|}{\textbf{DEFINITION}} &
%   \begin{tabular}[c]{@{}l@{}}low spirits ; depression <sep> wander about listlessly and \\ aimlessly because of unhappiness or boredom\end{tabular} \\ \midrule
% \multicolumn{1}{l|}{\textbf{SDM\_PRED}} &
%   \multicolumn{1}{l|}{the act of smoking <sep> a change of mind or attitude} &
%   \multicolumn{1}{l|}{\textbf{SDM\_PRED}} &
%   feel despondency <sep> an act of moping \\ \midrule
% \multicolumn{1}{l|}{\textbf{MDM\_PRED}} &
%   \multicolumn{1}{l|}{make ( something ) illegal <sep> prevent ( someone ) from doing something} &
%   \multicolumn{1}{l|}{\textbf{MDM\_PRED}} &
%   a period of unhappiness or unhappiness <sep> wander aimlessly \\ \bottomrule[2pt]
% \end{tabular}
% }
% \caption{This table listed generated definitions from BART-SDM and BART-MDM on incomplete datasets in Quantitative Analysis on Generated Multiple Definition.}
% \label{tabel_case_study}
% \end{table*}

% \begin{table*}[htbp]
% \renewcommand{\arraystretch}{0.9}
% \scalebox{0.52}{
% \begin{tabular}{@{}llll@{}}
% \toprule[2pt]
% \multicolumn{4}{c}{\textbf{DEL 1}} \\ \midrule
% \multicolumn{1}{l|}{\textbf{WORD}} &
%   \multicolumn{1}{l|}{japanese} &
%   \multicolumn{1}{l|}{\textbf{WORD}} &
%   submerse \\ \midrule
% \multicolumn{1}{l|}{\textbf{CONTEXT}} &
%   \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}<w> japanese <w> unlike the belgians , americans and japanese ,\\ the british have no heritage of adult comic books .\end{tabular}} &
%   \multicolumn{1}{l|}{\textbf{CONTEXT}} &
%   \begin{tabular}[c]{@{}l@{}}<w> submerse <w> this is one of the great strengths of the play ; \\ though it may at times seem over-determined , and perhaps even obvious , \\ the audience is entirely submersed in the characters and their worlds .\end{tabular} \\ \midrule
% \multicolumn{1}{l|}{\textbf{DEFINITION}} &
%   \multicolumn{1}{l|}{a native or inhabitant of japan , or a person of  japanese descent .} &
%   \multicolumn{1}{l|}{\textbf{DEFINITION}} &
%   submerge \\ \midrule
% \multicolumn{1}{l|}{\textbf{SDM\_PRED}} &
%   \multicolumn{1}{l|}{the mandarin language of japan.} &
%   \multicolumn{1}{l|}{\textbf{SDM\_PRED}} &
%   make rigid or rigid \\ \midrule
% \multicolumn{1}{l|}{\textbf{MDM\_PRED}} &
%   \multicolumn{1}{l|}{a native or inhabitant of japan.} &
%   \multicolumn{1}{l|}{\textbf{MDM\_PRED}} &
%   become immersed in \\ \midrule
% \multicolumn{4}{c}{\textbf{DEL 2}} \\ \midrule
% \multicolumn{1}{l|}{\textbf{WORD}} &
%   \multicolumn{1}{l|}{snitch} &
%   \multicolumn{1}{l|}{\textbf{WORD}} &
%   ban \\ \midrule
% \multicolumn{1}{l|}{\textbf{CONTEXT}} &
%   \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}<w> snitch <w> he believes in the value of student snitches , parental conferences , \\ and long hot showers in the faculty lounge . <sep> \\ trey kicked at it as he snitched a chocolate chip cookie from blake 's lunch .\end{tabular}} &
%   \multicolumn{1}{l|}{\textbf{CONTEXT}} &
%   \begin{tabular}[c]{@{}l@{}}<w> ban  <w> smoking is banned in this building  <sep>  the subject is \\ banned from our interview because the case has still to come to court .\end{tabular} \\ \midrule
% \multicolumn{1}{l|}{\textbf{DEFINITION}} &
%   \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}a hiding place sometimes used by hunters especially duck hunters \\ <sep> not based on reason or evidence\end{tabular}} &
%   \multicolumn{1}{l|}{\textbf{DEFINITION}} &
%   \begin{tabular}[c]{@{}l@{}}prohibit especially by legal means or social pressure \\ <sep> officially or legally prohibit ( something )\end{tabular} \\ \midrule
% \multicolumn{1}{l|}{\textbf{SDM\_PRED}} &
%   \multicolumn{1}{l|}{a person who is blind <sep> not aware of} &
%   \multicolumn{1}{l|}{\textbf{SDM\_PRED}} &
%   the act of smoking <sep> a change of mind or attitude \\ \midrule
% \multicolumn{1}{l|}{\textbf{MDM\_PRED}} &
%   \multicolumn{1}{l|}{unable to see <sep>  unable to perceive} &
%   \multicolumn{1}{l|}{\textbf{MDM\_PRED}} &
%   make ( something ) illegal <sep> prevent ( someone ) from doing something \\ \bottomrule[2pt]
% \end{tabular}
% }
% \caption{This table listed generated definitions from BART-SDM and BART-MDM on incomplete datasets in Quantitative Analysis on Generated Multiple Definition.}
% \label{tabel_case_study}
% \end{table*}

\begin{table}[htbp]
\renewcommand{\arraystretch}{0.9}
\scalebox{0.52}{
\begin{tabular}{@{}llll@{}}
\toprule[2pt]
\multicolumn{2}{c}{\textbf{DEL 1}}                                                                                  \\ \midrule
\multicolumn{1}{l|}{\textbf{WORD}}       & japanese                                                                 \\ \midrule
\multicolumn{1}{l|}{\textbf{CONTEXT}} &
  \begin{tabular}[c]{@{}l@{}}w japanese w unlike the belgians , americans and japanese ,\\ the british have no heritage of adult comic books .\end{tabular} \\ \midrule
\multicolumn{1}{l|}{\textbf{DEFINITION}} & a native or inhabitant of japan , or a person of  japanese descent .     \\ \midrule
\multicolumn{1}{l|}{\textbf{SDM\_PRED}}  & the mandarin language of japan.                                          \\ \midrule
\multicolumn{1}{l|}{\textbf{MDM\_PRED}}  & a native or inhabitant of japan.                                         \\ \midrule
\multicolumn{2}{c}{\textbf{DEL 2}}                                                                                  \\ \midrule
\multicolumn{1}{l|}{\textbf{WORD}}       & ban                                                                      \\ \midrule
\multicolumn{1}{l|}{\textbf{CONTEXT}} &
  \begin{tabular}[c]{@{}l@{}}w ban  w smoking is banned in this building  sep  the subject is \\ banned from our interview because the case has still to come to court .\end{tabular} \\ \midrule
\multicolumn{1}{l|}{\textbf{DEFINITION}} &
  \begin{tabular}[c]{@{}l@{}}prohibit especially by legal means or social pressure \\ sep  officially or legally prohibit ( something )\end{tabular} \\ \midrule
\multicolumn{1}{l|}{\textbf{SDM\_PRED}}  & the act of smoking sep a change of mind or attitude                      \\ \midrule
\multicolumn{1}{l|}{\textbf{MDM\_PRED}}  & make ( something ) illegal sep  prevent ( someone ) from doing something \\ \bottomrule[2pt]
\end{tabular}
}
\caption{Examples of generated definitions from BART-SDM and BART-MDM on DEL-$D$ datasets with an incomplete sense inventory.}
\label{tabel_case_study}
\end{table}
